Steganography: a Class of Algorithms having Secure Properties

Chaos-based approaches are frequently proposed in information hiding, but without obvious justification. Indeed, the reason why chaos is useful to tackle with discretion, robustness, or security, is rarely elucidated. This research work presents a new class of non-blind information hidingalgorithms based on some finite domains iterations that are Devaney's topologically chaotic. The approach is entirely formalized and reasons to take place into the mathematical theory of chaos are explained. Finally, stego-security and chaos security are consequently proven for a large class of algorithms.

==> attacks.tex <==



As far as we know, Cachin~\cite{Cachin2004}
produces the first fundamental work in information hiding security:
in the context of steganography, the attempt of an attacker to distinguish 
between an innocent image and a stego-content is viewed as a hypothesis 
testing problem.
Mittelholzer~\cite{Mittelholzer99}, next proposed the first theoretical 
framework for analyzing the security of a watermarking scheme.
Clarification between  robustness and security 
and classifications of watermarking attacks
have been firstly presented by Kalker~\cite{Kalker2001}.
This work has been deepened by Furon \emph{et al.}~\cite{Furon2002}, who have translated Kerckhoffs' principle (Alice and Bob shall only rely on some previously shared secret for privacy), from cryptography to data hiding. 

More recently~\cite{Cayre2005,Perez06} classified the information hiding  
attacks into categories, according to the type of information the attacker (Eve)
has access to:
\begin{itemize}
\item in Watermarked Only Attack (WOA) she only knows embedded contents $z$;
\item in Known Message Attack (KMA) she knows pairs $(z,y)$ of embedded
  contents and corresponding messages;
\item in Known Original Attack (KOA) she knows several pairs $(z,x)$ 
  of embedded contents and their corresponding original versions;
\item in Constant-Message Attack (CMA) she observes several embedded
  contents $z_1$,\ldots,$z_k$ and only knows that the unknown 
  hidden message $y$ is the same in all contents.
\end{itemize}

To the best of our knowledge, 
KMA, KOA, and CMA have not already been studied
due to the lack of theoretical framework.
In the opposite, security of data hiding against WOA can be evaluated,
by using a probabilistic approach recalled below.





==> dct.tex <==
Let us denote by $x$ the orignal image of size $H \times L$, and by $y$
the hidden message, supposed here to be a binary image of size $H' \times L'$. %
The image $x$ is transformed from the spatial
domain to DCT domain frequency bands,
in order to embed $y$ inside it.  
To do so, the host image is firstly divided into $8 \times 8$
image blocks as given below:
$$x = \bigcup_{k=1}^{H/8} \bigcup_{k'=1}^{L/8} x(k,k').$$
Thus, for each image block,
DCT is performed and the coefficients in the frequency bands 
are obtained as follows:
$x_{DCT}(m;n) = DCT(x(m;n))$.

To define a discrete but robust scheme, only the four following coefficients of each $8 \times 8$ block in position $(m,n)$ will be eventually modified: $x_{DCT}(m;n)_{(3,1)},$ $x_{DCT}(m;n)_{(2,2)},$ or $x_{DCT}(m;n)_{(1,3)}$. This choice can be reformulated as follows. 
Coefficients of each DCT matrix are re-indexed by using a diagonal southwest/northeast diagonal, such that $i_{DCT}(m,n)_1 = x_{DCT}(m;n)_{(1,1)}$,\linebreak $i_{DCT}(m,n)_2 = x_{DCT}(m;n)_{(2,1)}$, $i_{DCT}(m,n)_3 = x_{DCT}(m;n)_{(1,2)}$, $i_{DCT}(m,n)_4 = x_{DCT}(m;n)_{(3,1)}$, ..., and $i_{DCT}(m,n)_{64} =$  $ x_{DCT}(m;n)_{(8,8)}$.
So the signification function can be defined in this context by:
\begin{itemize}
\item if $k$ mod $64 \in \{1,2,3\}$ and $k\leqslant H\times L$, then $u^k=1$,
\item else if $k$ mod $64 \in \{4, 5, 6\}$ and $k\leqslant H\times L$, then $u^k=-1$,
\item else $u^k = 0$.
\end{itemize}
The significance of coefficients are obtained for instance with $m=-0.5$ and $M=0.5$, leading to the definitions of MSCs, LSCs, and passive coefficients.
Thus, decomposition and recomposition functions are fully defined and dhCI dissimulation scheme can now be applied.

In that situation and with the same parameters than in the previous section, we found a RMS equal to 1.731.



==> discussion.tex <==

Thus only a  binary information can finally be embedded into  a given host, when
using  the  \emph{dhCI dissimulation}  algorithm:  hidden  message  $y$ is  more
related  to a  private  embedding  key. Moreover,  this  data hiding scheme  is
non-blind  as  the  original host  is  required  to  extract the  binary  hidden
information.  These two  strong requirements  can lead  to the  belief  that the
\emph{dhCI dissimulation} is finally not  really helpful in most situations that
occur in information hiding.



Furthermore,  enlarging the given payload  of a data  hiding scheme leads
clearly to  a degradation of its  security: the smallest the  number of embedded
bits is, the better the security is. Additionally, this scheme can be adapted to
situations where  security is not a  strong requirement, as  follows. Instead of
realizing  chaotic iterations  on  LSCs, it  is  also possible  to replace  bits
selected  by  the  chaotic strategy  with  those  of  the hidden  message.  This
replacement (in place of the switch)  leads to the ability to extract the hidden
bits, but the security of the scheme is consequently reduced to the sole chaotic
selection of LSCs.



==> dwt.tex <==

Let us now explain how the dhCI dissimulation can be applied in the discrete wavelets domain (DWT).
In this paper, the Daubechies family of wavelets is chosen: 
a bitmap file of the famous Lena is converted into its Daubechies-1 DWT
coefficients, which are altered by chaotic iterations. 

Each DWT decomposition depends on a decomposition level and a coefficient
matrix (Figure~\ref{fig:DWTs}): $\textit{LL}$ means approximation coefficient,
when $\textit{HH},\textit{LH},\textit{HL}$ denote respectively diagonal, vertical and horizontal detail coefficients. 
For example, the DWT coefficient \textit{HH}2 is the matrix equal to the diagonal detail coefficient of the second level of decomposition of Lena.

\begin{figure}[htb]
\centerline{\epsfig{figure=DWTs.pdf,width=3.7cm}}
\caption{Wavelets coefficients.}
\label{fig:DWTs}
\end{figure}

Let us now explain how to use the dhCI algorithm in a context of \{\textit{HL}2,\textit{HH}2,\textit{LH}2\}-embedding after 3 levels of decomposition.

We suppose that Lena has $2^k \times 2^k$ pixels.
Each DWT coefficient $\textit{LL}1$, $\textit{LL}2$\ldots$\textit{HL}3$  
of size $2^{k-i}\times 2^{k-i}$ is put into a matrix $W$ as it is depicted in in Figure \ref{fig:DWTs}.
We reindex this matrix block after block, following a southwest-northeast direction, such that:
\begin{itemize}
\item $W_1 = \textit{LL}3_{(1,1)}$, $W_2 = \textit{LL}3_{(2,1)}$, $W_3 = \textit{LL}3_{(1,2)}$, ..., $W_{2^{k-3}\times 2^{k-3}} = \textit{LL}3_{(2^{k-3}, 2^{k-3})}$,
\item $W_{2^{k-3}\times 2^{k-3}+1} = \textit{LH}3_{(1,1)}$, $W_{2^{k-3}\times 2^{k-3}+2} = \textit{LH}3_{(2,1)}$, $W_{2^{k-3}\times 2^{k-3}+3} = \textit{LH}3_{(1,2)}$, ..., $W_{2 \times 2^{k-3}\times 2^{k-3}} = \textit{LH}3_{(2^{k-3}, 2^{k-3})}$,
\item $W_{2\times 2^{k-3}\times 2^{k-3}+1} = \textit{HL}3_{(1,1)}$, $W_{2\times 2^{k-3}\times 2^{k-3}+2} = \textit{HL}3_{(2,1)}$, $W_{2\times 2^{k-3}\times 2^{k-3}+3} = \textit{HL}3_{(1,2)}$, ..., $W_{3 \times 2^{k-3}\times 2^{k-3}} = \textit{HL}3_{(2^{k-3}, 2^{k-3})}$,
\item $W_{3\times 2^{k-3}\times 2^{k-3}+1} = \textit{HH}3_{(1,1)}$, $W_{3\times 2^{k-3}\times 2^{k-3}+2} = \textit{HH}3_{(2,1)}$, $W_{3\times 2^{k-3}\times 2^{k-3}+3} = \textit{HH}3_{(1,2)}$, ..., $W_{2^{k-2}\times 2^{k-2}} = \textit{HH}3_{(2^{k-3}, 2^{k-3})}$,
\item etc.
\end{itemize}
Thus a definition of a decomposition function $u$ can be:
\begin{itemize}
\item $u^k = 2$ if $k \leqslant 2^{k-3}\times 2^{k-3}$, 
\item $u^k = 1$ if $k \in \llbracket 2^{k-3}\times 2^{k-3}+1, 2^{k-2}\times 2^{k-2} \rrbracket$,
\item $u^k = -1$ if $k \in \llbracket 2^{k-2}\times 2^{k-2}+1, 2^{k-1}\times 2^{k-1} \rrbracket$,
\item else $u^k = 0$.
\end{itemize}

The significance of coefficients are obtained for instance with $m=-0.5$ and $M=1.5$, leading to the definitions of MSCs = \textit{LL}3 and LSCs = \{\textit{HL}2,\textit{HH}2,\textit{LH}2\}.
Thus, decomposition and recomposition functions are fully defined and dhCI dissimulation scheme can now be applied.

Figure \ref{fig:DWT} shows the result of a dhCI dissimulation embedding into DWT domain by using a configuration as above. CIIS is the strategy-adapter ($K=0.12345, \alpha=0.25$, $y$ is given in Figure \ref{(b) Watermark}, and $l=1000$) and the vectorial negation is the chosen mode of this dissimulation (PSNR : 53.765).

\begin{figure}[h]
  \centering
  \subfigure[Original Lena.]{\includegraphics[width=0.24\textwidth]{lena512.jpg}\label{(a) Original Lena}}\hspace{1cm}
  \subfigure[$k$]{\includegraphics[width=0.08\textwidth]{invader.png}\label{(b) Watermark}}\hspace{1cm}
  \subfigure[Modified Lena.]{\includegraphics[width=0.24\textwidth]{lena512marque.png}\label{(b) Watermarked Lena}}
\caption{Data hiding in DWT domain}
\label{fig:DWT}
\end{figure}


The classical RMS error value defined by 
$\sqrt{\frac{1}{n}\sum_{k=1}^n{(x-z)_k^2}}$ 
is computed to evaluate the differences.
  The probability that the image contains hidden message   
 increases when the RMS decreases.
In that situation, we found a RMS equal to 1.016.

